Lean-Quantum: Toward AI-Assisted Formalization of Quantum Information

Quantum information theory is built on entropic quantities; among them, the sandwiched R\'enyi relative entropy is a fundamental divergence with various applications, and its data processing inequality (DPI) under quantum channels is a cornerstone result. In this work, we present a Lean 4 library for quantum information, designed as a reusable formal infrastructure for theoretical analysis. As a central demonstration of the library, we formalize the DPI for the sandwiched R\'enyi relative entropy for positive semidefinite operators on finite-dimensional quantum systems. The library provides a basis-independent operator-theoretic framework for finite-dimensional quantum mechanics compatible with the standard mathematical library Mathlib, including reusable interfaces for finite-dimensional systems, states, channels, tensor products, partial traces, Choi operators, Kraus representations, and Stinespring representations. It also builds infrastructure for noncommutative trace inequalities, including operator monotonicity and convexity via the real continuous functional calculus, block-operator positivity, Hilbert-Schmidt operator spaces, Jensen's operator inequality, generalized perspectives, operator power means, and Lieb-Ando trace inequalities. On top of this framework, we formalize entropy-specific ingredients for the DPI: variational formulas for the sandwiched quasi-entropy via Young and reverse-Young inequalities, tensor-product compatibility of real powers, and Haar measures on unitary groups. Together, these components yield a Lean formalization of the DPI, give strong subadditivity as a corollary, and provide the last missing component needed to complete the Lean formalization of the generalized quantum Stein's lemma. More broadly, the development provides machine-checkable foundations for future formalized and AI-assisted research in quantum information theory.

==> lstlean.tex <==
\lstdefinelanguage{lean}{
  % Keywords
  morekeywords=[1]{
    import, prelude, protected, private, noncomputable, definition, meta, 
    renaming, hiding, parameter, parameters, begin, constant, constants, 
    lemma, variable, variables, theory, print, theorem, example, open, 
    as, export, override, axiom, axioms, inductive, with, structure, 
    record, universe, universes, alias, help, precedence, reserve, 
    declare_trace, add_key_equivalence, match, infix, infixl, infixr, 
    notation, postfix, prefix, instance, eval, reduce, check, end, 
    this, using, using_well_founded, namespace, section, attribute, 
    local, set_option, extends, include, omit, class, raw, replacing, 
    calc, have, show, suffices, by, in, at, let, forall, Pi, fun, 
    exists, if, dif, then, else, assume, obtain, from, register_simp_ext, 
    unless, break, continue, mutual, do, def, run_cmd, const, partial, 
    mut, where, macro, syntax, deriving, return, try, catch, for, 
    macro_rules, declare_syntax_cat, abbrev
  },
  % Sorts
  morekeywords=[2]{Sort, Type, Prop},
  % Tactics
  morekeywords=[3]{
    assumption, apply, intro, intros, allGoals, generalize, clear, 
    revert, done, exact, refine, repeat, cases, rewrite, rw, simp, 
    simp_all, contradiction, constructor, injection, induction
  },
  % Comments
  morecomment=[s][\color{commentcolor}]{/-}{-/},
  morecomment=[l][\color{commentcolor}]{--},
  % Strings
  morestring=[b]",
  % Style
  sensitive=true,
  breaklines=true,
  showstringspaces=false,
  basicstyle=\ttfamily,
  keywordstyle=[1]\color{keywordcolor}\bfseries,
  keywordstyle=[2]\color{sortcolor}\bfseries,
  keywordstyle=[3]\color{tacticcolor}\bfseries,
  commentstyle=\itshape\color{commentcolor},
  stringstyle=\color{stringcolor},
  % Unicode replacements (Literate programming)
  literate=
    {α}{{\ensuremath{\alpha}}}1
    {β}{{\ensuremath{\beta}}}1
    {γ}{{\ensuremath{\gamma}}}1
    {δ}{{\ensuremath{\delta}}}1
    {ε}{{\ensuremath{\epsilon}}}1
    {ζ}{{\ensuremath{\zeta}}}1
    {η}{{\ensuremath{\eta}}}1
    {θ}{{\ensuremath{\theta}}}1
    {ι}{{\ensuremath{\iota}}}1
    {κ}{{\ensuremath{\kappa}}}1
    {μ}{{\ensuremath{\mu}}}1
    {ν}{{\ensuremath{\nu}}}1
    {ξ}{{\ensuremath{\xi}}}1
    {π}{{\ensuremath{\pi}}}1
    {ρ}{{\ensuremath{\rho}}}1
    {σ}{{\ensuremath{\sigma}}}1
    {τ}{{\ensuremath{\tau}}}1
    {υ}{{\ensuremath{\upsilon}}}1
    {φ}{{\ensuremath{\phi}}}1
    {χ}{{\ensuremath{\chi}}}1
    {ψ}{{\ensuremath{\psi}}}1
    {ω}{{\ensuremath{\omega}}}1
    {Γ}{{\ensuremath{\Gamma}}}1
    {Δ}{{\ensuremath{\Delta}}}1
    {Θ}{{\ensuremath{\Theta}}}1
    {Λ}{{\ensuremath{\Lambda}}}1
    {Σ}{{\ensuremath{\Sigma}}}1
    {Φ}{{\ensuremath{\Phi}}}1
    {Ξ}{{\ensuremath{\Xi}}}1
    {Ψ}{{\ensuremath{\Psi}}}1
    {Ω}{{\ensuremath{\Omega}}}1
    {≤}{{\ensuremath{\le}}}1
    {≥}{{\ensuremath{\ge}}}1
    {≠}{{\ensuremath{\ne}}}1
    {≈}{{\ensuremath{\approx}}}1
    {≡}{{\ensuremath{\equiv}}}1
    {≃}{{\ensuremath{\simeq}}}1
    {∧}{{\ensuremath{\wedge}}}1
    {∨}{{\ensuremath{\vee}}}1
    {¬}{{\ensuremath{\neg}}}1
    {⊢}{{\ensuremath{\vdash}}}1
    {⟨}{{\ensuremath{\langle}}}1
    {⟩}{{\ensuremath{\rangle}}}1
    {↦}{{\ensuremath{\mapsto}}}1
    {←}{{\ensuremath{\leftarrow}}}1
    {→}{{\ensuremath{\to}}}1
    {↔}{{\ensuremath{\leftrightarrow}}}1
    {⇒}{{\ensuremath{\Rightarrow}}}1
    {⟹}{{\ensuremath{\Longrightarrow}}}1
    {⇐}{{\ensuremath{\Leftarrow}}}1
    {⟸}{{\ensuremath{\Longleftarrow}}}1
    {∩}{{\ensuremath{\cap}}}1
    {∪}{{\ensuremath{\cup}}}1
    {⊂}{{\ensuremath{\subset}}}1
    {⊆}{{\ensuremath{\subseteq}}}1
    {⊃}{{\ensuremath{\supset}}}1
    {⊇}{{\ensuremath{\supseteq}}}1
    {∈}{{\ensuremath{\in}}}1
    {∉}{{\ensuremath{\notin}}}1
    {∋}{{\ensuremath{\ni}}}1
    {∅}{{\ensuremath{\emptyset}}}1
    {ℕ}{{\ensuremath{\mathbb{N}}}}1
    {ℤ}{{\ensuremath{\mathbb{Z}}}}1
    {ℝ}{{\ensuremath{\mathbb{R}}}}1
    {ℚ}{{\ensuremath{\mathbb{Q}}}}1
    {ℂ}{{\ensuremath{\mathbb{C}}}}1
    {∀}{{\ensuremath{\forall}}}1
    {∃}{{\ensuremath{\exists}}}1
    {λ}{{\ensuremath{\lambda}}}1
    {:=}{{:}{=}}2
    {==}{{=}{=}}2
    {++}{{+}{+}}2
    {·}{{\ensuremath{\cdot}}}1
    {▸}{{\ensuremath{\blacktriangleright}}}1
    {⊗}{{\ensuremath{\otimes}}}1
    {†}{{\ensuremath{^\dagger}}}1
    {‖}{{\ensuremath{\Vert}}}1
    {×}{{\ensuremath{\times}}}1
    {ˢ}{{\ensuremath{^s}}}1
    {¹}{{\ensuremath{^1}}}1
    {⁻¹}{{\ensuremath{^{-1}}}}1
    {₁}{{\ensuremath{_1}}}1
    {₂}{{\ensuremath{_2}}}1
    {₃}{{\ensuremath{_3}}}1
    {ₐ}{{\ensuremath{_a}}}1
    {ₗ}{{\ensuremath{_l}}}1
    {ₜ}{{\ensuremath{_t}}}1
    {ℋ}{{\ensuremath{\mathcal{H}}}}1
    {ℋ₁}{{\ensuremath{\mathcal{H}_1}}}2
    {ℋ₂}{{\ensuremath{\mathcal{H}_2}}}2
    {ℋ₃}{{\ensuremath{\mathcal{H}_3}}}2
    {��}{{\ensuremath{\mathcal{A}}}}1
    {→ₗ}{{\ensuremath{\to_l}}}2
    {∘ₗ}{{\ensuremath{\circ_l}}}2
    {∘}{{\ensuremath{\circ}}}1
    {⋆}{{\ensuremath{\star}}}1
    {•}{{\ensuremath{\cdot}}}1
    {∫}{{\ensuremath{\int}}}1
    {∂}{{\ensuremath{\partial}}}1
    {∑}{{\ensuremath{\sum}}}1
    {⨆}{{\ensuremath{\bigsqcup}}}1
    {⦃}{{\ensuremath{\lbrace}}}1
    {⦄}{{\ensuremath{\rbrace}}}1
    {ⁿ}{{\ensuremath{^n}}}1
    {Tr}{{\ensuremath{\Tr}}}2
    {dinv}{{\ensuremath{\dimHinv}}}4
    {dim}{{\ensuremath{\dimH}}}3

    {ᵐ}{{\ensuremath{^m}}}1
    {ᵤ}{{\ensuremath{^u}}}1
    {ᵥ}{{\ensuremath{^v}}}1
    {ᵢ}{{\ensuremath{^i}}}1
    {ᵣ}{{\ensuremath{^r}}}1
    {ᵦ}{{\ensuremath{^\beta}}}1
    {��}{{\ensuremath{\mathcal{K}}}}1
    {��}{{\ensuremath{\mathcal{A}}}}1
    {��}{{\ensuremath{\mathcal{B}}}}1
    {��}{{\ensuremath{\mathcal{J}}}}1
    {��}{{\ensuremath{\mathcal{X}}}}1
    {��}{{\ensuremath{\mathcal{P}}}}1
    {⋯}{{\ensuremath{\cdots}}}1
}

